Highlights from the Pierre Auger Observatory (ICRC17)

In this contribution we summarize the highlights from the Pierre Auger Observatory presented at the 35th International Cosmic Ray Conference. We discuss the update of the measurement of the energy spectrum of cosmic rays over a wide range of energy ($10^{17.5}$ to above $10^{20}$ eV), studies of the cosmic-ray mass composition with the fluorescence and surface detector of the Observatory, the discovery of a large-scale anisotropy in the arrival direction of cosmic rays above $8\times 10^{18}$ eV and indications of anisotropy at intermediate angular scales above $4 \times 10^{19}$ eV. Moreover, we report on tests of hadronic interactions beyond LHC energies, multi-messenger analyses with neutral primaries and the progress of the upgrade of the Observatory, AugerPrime, aimed at elucidating the origin of the observed flux suppression at ultra-high energies.

==> acknowledgments.tex <==
% created on 2017-08-14

\section*{Acknowledgments}

\begin{sloppypar}
The successful installation, commissioning, and operation of the Pierre
Auger Observatory would not have been possible without the strong
commitment and effort from the technical and administrative staff in
Malarg\"ue. We are very grateful to the following agencies and
organizations for financial support:
\end{sloppypar}

\begin{sloppypar}
Argentina -- Comisi\'on Nacional de Energ\'\i{}a At\'omica; Agencia Nacional de
Promoci\'on Cient\'\i{}fica y Tecnol\'ogica (ANPCyT); Consejo Nacional de
Investigaciones Cient\'\i{}ficas y T\'ecnicas (CONICET); Gobierno de la
Provincia de Mendoza; Municipalidad de Malarg\"ue; NDM Holdings and Valle
Las Le\~nas; in gratitude for their continuing cooperation over land
access; Australia -- the Australian Research Council; Brazil -- Conselho
Nacional de Desenvolvimento Cient\'\i{}fico e Tecnol\'ogico (CNPq);
Financiadora de Estudos e Projetos (FINEP); Funda\c{c}\~ao de Amparo \`a
Pesquisa do Estado de Rio de Janeiro (FAPERJ); S\~ao Paulo Research
Foundation (FAPESP) Grants No.~2010/07359-6 and No.~1999/05404-3;
Minist\'erio de Ci\^encia e Tecnologia (MCT); Czech Republic -- Grant
No.~MSMT CR LG15014, LO1305, LM2015038 and
CZ.02.1.01/0.0/0.0/16\_013/0001402; France -- Centre de Calcul
IN2P3/CNRS; Centre National de la Recherche Scientifique (CNRS); Conseil
R\'egional Ile-de-France; D\'epartement Physique Nucl\'eaire et Corpusculaire
(PNC-IN2P3/CNRS); D\'epartement Sciences de l'Univers (SDU-INSU/CNRS);
Institut Lagrange de Paris (ILP) Grant No.~LABEX ANR-10-LABX-63 within
the Investissements d'Avenir Programme Grant No.~ANR-11-IDEX-0004-02;
Germany -- Bundesministerium f\"ur Bildung und Forschung (BMBF); Deutsche
Forschungsgemeinschaft (DFG); Finanzministerium Baden-W\"urttemberg;
Helmholtz Alliance for Astroparticle Physics (HAP);
Helmholtz-Gemeinschaft Deutscher Forschungszentren (HGF); Ministerium
f\"ur Innovation, Wissenschaft und Forschung des Landes
Nordrhein-Westfalen; Ministerium f\"ur Wissenschaft, Forschung und Kunst
des Landes Baden-W\"urttemberg; Italy -- Istituto Nazionale di Fisica
Nucleare (INFN); Istituto Nazionale di Astrofisica (INAF); Ministero
dell'Istruzione, dell'Universit\'a e della Ricerca (MIUR); CETEMPS Center
of Excellence; Ministero degli Affari Esteri (MAE); Mexico -- Consejo
Nacional de Ciencia y Tecnolog\'\i{}a (CONACYT) No.~167733; Universidad
Nacional Aut\'onoma de M\'exico (UNAM); PAPIIT DGAPA-UNAM; The Netherlands
-- Ministerie van Onderwijs, Cultuur en Wetenschap; Nederlandse
Organisatie voor Wetenschappelijk Onderzoek (NWO); Stichting voor
Fundamenteel Onderzoek der Materie (FOM); Poland -- National Centre for
Research and Development, Grants No.~ERA-NET-ASPERA/01/11 and
No.~ERA-NET-ASPERA/02/11; National Science Centre, Grants
No.~2013/08/M/ST9/00322, No.~2013/08/M/ST9/00728 and No.~HARMONIA
5--2013/10/M/ST9/00062, UMO-2016/22/M/ST9/00198; Portugal -- Portuguese
national funds and FEDER funds within Programa Operacional Factores de
Competitividade through Funda\c{c}\~ao para a Ci\^encia e a Tecnologia
(COMPETE); Romania -- Romanian Authority for Scientific Research ANCS;
CNDI-UEFISCDI partnership projects Grants No.~20/2012 and No.~194/2012
and PN 16 42 01 02; Slovenia -- Slovenian Research Agency; Spain --
Comunidad de Madrid; Fondo Europeo de Desarrollo Regional (FEDER) funds;
Ministerio de Econom\'\i{}a y Competitividad; Xunta de Galicia; European
Community 7th Framework Program Grant No.~FP7-PEOPLE-2012-IEF-328826;
USA -- Department of Energy, Contracts No.~DE-AC02-07CH11359,
No.~DE-FR02-04ER41300, No.~DE-FG02-99ER41107 and No.~DE-SC0011689;
National Science Foundation, Grant No.~0450696; The Grainger Foundation;
Marie Curie-IRSES/EPLANET; European Particle Physics Latin American
Network; European Union 7th Framework Program, Grant
No.~PIRSES-2009-GA-246806; European Union's Horizon 2020 research and
innovation programme (Grant No.~646623); and UNESCO.
\end{sloppypar}


==> icrc2017_authors.tex <==
% created on 2017-07-31

A.~Aab$^{77}$,
P.~Abreu$^{69}$,
M.~Aglietta$^{50,49}$,
I.F.M.~Albuquerque$^{18}$,
I.~Allekotte$^{1}$,
A.~Almela$^{8,11}$,
J.~Alvarez Castillo$^{65}$,
J.~Alvarez-Mu\~niz$^{76}$,
G.A.~Anastasi$^{41,43}$,
L.~Anchordoqui$^{83}$,
B.~Andrada$^{8}$,
S.~Andringa$^{69}$,
C.~Aramo$^{47}$,
N.~Arsene$^{71}$,
H.~Asorey$^{1,27}$,
P.~Assis$^{69}$,
J.~Aublin$^{32}$,
G.~Avila$^{9,10}$,
A.M.~Badescu$^{72}$,
A.~Balaceanu$^{70}$,
F.~Barbato$^{57}$,
R.J.~Barreira Luz$^{69}$,
K.H.~Becker$^{34}$,
J.A.~Bellido$^{12}$,
C.~Berat$^{33}$,
M.E.~Bertaina$^{59,49}$,
X.~Bertou$^{1}$,
P.L.~Biermann$^{b}$,
J.~Biteau$^{31}$,
S.G.~Blaess$^{12}$,
A.~Blanco$^{69}$,
J.~Blazek$^{29}$,
C.~Bleve$^{53,45}$,
M.~Boh\'a\v{c}ov\'a$^{29}$,
D.~Boncioli$^{43,g}$, %added
C.~Bonifazi$^{24}$,
N.~Borodai$^{66}$,
A.M.~Botti$^{8,36}$,
J.~Brack$^{f}$,
I.~Brancus$^{70}$,
T.~Bretz$^{38}$,
A.~Bridgeman$^{35}$,
F.L.~Briechle$^{38}$,
P.~Buchholz$^{40}$,
A.~Bueno$^{75}$,
S.~Buitink$^{77}$,
M.~Buscemi$^{55,44}$,
K.S.~Caballero-Mora$^{63}$,
B.~Caccianiga$^{46}$, %added
L.~Caccianiga$^{56}$,
A.~Cancio$^{11,8}$,
F.~Canfora$^{77}$,
L.~Caramete$^{71}$,
R.~Caruso$^{55,44}$,
A.~Castellina$^{50,49}$,
F.~Catalani$^{16}$, % change 18-->16
G.~Cataldi$^{45}$,
L.~Cazon$^{69}$,
A.G.~Chavez$^{64}$,
J.A.~Chinellato$^{19}$,
J.~Chudoba$^{29}$,
R.W.~Clay$^{12}$,
A.~Cobos$^{8}$,
R.~Colalillo$^{57,47}$,
A.~Coleman$^{87}$,
L.~Collica$^{49}$,
M.R.~Coluccia$^{53,45}$,
R.~Concei\c{c}\~ao$^{69}$,
G.~Consolati$^{46}$,
G.~Consolati$^{46,51}$,
F.~Contreras$^{9,10}$,
M.J.~Cooper$^{12}$,
S.~Coutu$^{87}$,
C.E.~Covault$^{81}$,
J.~Cronin$^{88}$,
S.~D'Amico$^{52,45}$,
B.~Daniel$^{19}$,
S.~Dasso$^{5,3}$,
K.~Daumiller$^{36}$,
B.R.~Dawson$^{12}$,
R.M.~de Almeida$^{26}$,
S.J.~de Jong$^{77,79}$,
G.~De Mauro$^{77}$,
J.R.T.~de Mello Neto$^{24,25}$,
I.~De Mitri$^{53,45}$,
J.~de Oliveira$^{26}$,
V.~de Souza$^{17}$,
J.~Debatin$^{35}$,
O.~Deligny$^{31}$,
M.L.~D\'\i{}az Castro$^{19}$,
F.~Diogo$^{69}$,
C.~Dobrigkeit$^{19}$,
J.C.~D'Olivo$^{65}$,
Q.~Dorosti$^{40}$,
R.C.~dos Anjos$^{23}$,
M.T.~Dova$^{4}$,
A.~Dundovic$^{39}$,
J.~Ebr$^{29}$,
R.~Engel$^{36}$,
M.~Erdmann$^{38}$,
M.~Erfani$^{40}$,
C.O.~Escobar$^{e}$,
J.~Espadanal$^{69}$,
A.~Etchegoyen$^{8,11}$,
H.~Falcke$^{77,80,79}$,
J.~Farmer$^{88}$,
G.~Farrar$^{85}$,
A.C.~Fauth$^{19}$,
N.~Fazzini$^{e}$,
F.~Fenu$^{59,49}$,
B.~Fick$^{84}$,
J.M.~Figueira$^{8}$,
A.~Filip\v{c}i\v{c}$^{74,73}$,
M.M.~Freire$^{6}$,
T.~Fujii$^{88}$,
A.~Fuster$^{8,11}$,
R.~Ga\"\i{}or$^{32}$,
B.~Garc\'\i{}a$^{7}$,
F.~Gat\'e$^{d}$,
H.~Gemmeke$^{37}$,
A.~Gherghel-Lascu$^{70}$,
P.L.~Ghia$^{31}$,
U.~Giaccari$^{24}$,
M.~Giammarchi$^{46}$,
M.~Giller$^{67}$,
D.~G\l{}as$^{68}$,
C.~Glaser$^{38}$,
G.~Golup$^{1}$,
M.~G\'omez Berisso$^{1}$,
P.F.~G\'omez Vitale$^{9,10}$,
N.~Gonz\'alez$^{8,36}$,
A.~Gorgi$^{50,49}$,
A.F.~Grillo$^{43}$,
T.D.~Grubb$^{12}$,
F.~Guarino$^{57,47}$,
G.P.~Guedes$^{20}$,
R.~Halliday$^{81}$,
M.R.~Hampel$^{8}$,
P.~Hansen$^{4}$,
D.~Harari$^{1}$,
T.A.~Harrison$^{12}$,
A.~Haungs$^{36}$,
T.~Hebbeker$^{38}$,
D.~Heck$^{36}$,
P.~Heimann$^{40}$,
A.E.~Herve$^{35}$,
G.C.~Hill$^{12}$,
C.~Hojvat$^{e}$,
E.~Holt$^{36,8}$,
P.~Homola$^{66}$,
J.R.~H\"orandel$^{77,79}$,
P.~Horvath$^{30}$,
M.~Hrabovsk\'y$^{30}$,
T.~Huege$^{36}$,
J.~Hulsman$^{8,36}$,
A.~Insolia$^{55,44}$,
P.G.~Isar$^{71}$,
I.~Jandt$^{34}$,
J.A.~Johnsen$^{82}$,
M.~Josebachuili$^{8}$,
J.~Jurysek$^{29}$,
A.~K\"a\"ap\"a$^{34}$,
O.~Kambeitz$^{35}$,
K.H.~Kampert$^{34}$,
B.~Keilhauer$^{36}$,
N.~Kemmerich$^{18}$,
E.~Kemp$^{19}$,
J.~Kemp$^{38}$,
R.M.~Kieckhafer$^{84}$,
H.O.~Klages$^{36}$,
M.~Kleifges$^{37}$,
J.~Kleinfeller$^{9}$,
R.~Krause$^{38}$,
N.~Krohm$^{34}$,
D.~Kuempel$^{34}$, % change 38-->34
G.~Kukec Mezek$^{73}$,
N.~Kunka$^{37}$,
A.~Kuotb Awad$^{35}$,
B.L.~Lago$^{15}$,
D.~LaHurd$^{81}$,
R.G.~Lang$^{17}$,
M.~Lauscher$^{38}$,
R.~Legumina$^{67}$,
M.A.~Leigui de Oliveira$^{22}$,
A.~Letessier-Selvon$^{32}$,
I.~Lhenry-Yvon$^{31}$,
K.~Link$^{35}$,
D.~Lo Presti$^{55}$,
L.~Lopes$^{69}$,
R.~L\'opez$^{60}$,
A.~L\'opez Casado$^{76}$,
R.~Lorek$^{81}$,
Q.~Luce$^{31}$,
A.~Lucero$^{8,11}$,
M.~Malacari$^{88}$,
M.~Mallamaci$^{56,46}$,
D.~Mandat$^{29}$,
P.~Mantsch$^{e}$,
A.G.~Mariazzi$^{4}$,
I.C.~Mari\c{s}$^{13}$,
G.~Marsella$^{53,45}$,
D.~Martello$^{53,45}$,
H.~Martinez$^{61}$,
O.~Mart\'\i{}nez Bravo$^{60}$,
J.J.~Mas\'\i{}as Meza$^{3}$,
H.J.~Mathes$^{36}$,
S.~Mathys$^{34}$,
G.~Matthiae$^{58,48}$,
E.~Mayotte$^{34}$,
P.O.~Mazur$^{e}$,
C.~Medina$^{82}$,
G.~Medina-Tanco$^{65}$,
D.~Melo$^{8}$,
A.~Menshikov$^{37}$,
K.-D.~Merenda$^{82}$,
S.~Michal$^{30}$,
M.I.~Micheletti$^{6}$,
L.~Middendorf$^{38}$,
L.~Miramonti$^{56,46}$,
B.~Mitrica$^{70}$,
D.~Mockler$^{35}$,
S.~Mollerach$^{1}$,
F.~Montanet$^{33}$,
C.~Morello$^{50,49}$,
G.~Morlino$^{41,43}$,
M.~Mostaf\'a$^{87}$,
A.L.~M\"uller$^{8,36}$,
G.~M\"uller$^{38}$,
M.A.~Muller$^{19,21}$,
S.~M\"uller$^{35,8}$,
R.~Mussa$^{49}$,
I.~Naranjo$^{1}$,
L.~Nellen$^{65}$,
P.H.~Nguyen$^{12}$,
M.~Niculescu-Oglinzanu$^{70}$,
M.~Niechciol$^{40}$,
L.~Niemietz$^{34}$,
T.~Niggemann$^{38}$,
D.~Nitz$^{84}$,
D.~Nosek$^{28}$,
V.~Novotny$^{28}$,
L.~No\v{z}ka$^{30}$,
L.A.~N\'u\~nez$^{27}$,
L.~Ochilo$^{40}$,
F.~Oikonomou$^{87}$,
A.~Olinto$^{88}$,
M.~Palatka$^{29}$,
J.~Pallotta$^{2}$,
P.~Papenbreer$^{34}$,
G.~Parente$^{76}$,
A.~Parra$^{60}$,
T.~Paul$^{83}$,
M.~Pech$^{29}$,
F.~Pedreira$^{76}$,
J.~P\c{e}kala$^{66}$,
R.~Pelayo$^{62}$,
J.~Pe\~na-Rodriguez$^{27}$,
L.~A.~S.~Pereira$^{19}$,
M.~Perlin$^{8}$,
L.~Perrone$^{53,45}$,
C.~Peters$^{38}$,
S.~Petrera$^{41,43}$,
J.~Phuntsok$^{87}$,
R.~Piegaia$^{3}$,
T.~Pierog$^{36}$,
M.~Pimenta$^{69}$,
V.~Pirronello$^{55,44}$,
M.~Platino$^{8}$,
M.~Plum$^{38}$,
J.~Poh$^{88}$,
C.~Porowski$^{66}$,
R.R.~Prado$^{17}$,
P.~Privitera$^{88}$,
M.~Prouza$^{29}$,
E.J.~Quel$^{2}$,
S.~Querchfeld$^{34}$,
S.~Quinn$^{81}$,
R.~Ramos-Pollan$^{27}$,
J.~Rautenberg$^{34}$,
D.~Ravignani$^{8}$,
J.~Ridky$^{29}$,
F.~Riehn$^{69}$,
M.~Risse$^{40}$,
P.~Ristori$^{2}$,
V.~Rizi$^{54,43}$,
W.~Rodrigues de Carvalho$^{18}$,
G.~Rodriguez Fernandez$^{58,48}$,
J.~Rodriguez Rojo$^{9}$,
M.J.~Roncoroni$^{8}$,
M.~Roth$^{36}$,
E.~Roulet$^{1}$,
A.C.~Rovero$^{5}$,
P.~Ruehl$^{40}$,
S.J.~Saffi$^{12}$,
A.~Saftoiu$^{70}$,
F.~Salamida$^{54,43}$,
H.~Salazar$^{60}$,
A.~Saleh$^{73}$,
G.~Salina$^{48}$,
F.~S\'anchez$^{8}$,
P.~Sanchez-Lucas$^{75}$,
E.M.~Santos$^{18}$,
E.~Santos$^{8}$,
F.~Sarazin$^{82}$,
R.~Sarmento$^{69}$,
C.~Sarmiento-Cano$^{8}$,
R.~Sato$^{9}$,
M.~Schauer$^{34}$,
V.~Scherini$^{45}$,
H.~Schieler$^{36}$,
M.~Schimp$^{34}$,
D.~Schmidt$^{36,8}$,
O.~Scholten$^{78,c}$,
P.~Schov\'anek$^{29}$,
F.G.~Schr\"oder$^{36}$,
S.~Schr\"oder$^{34}$,
A.~Schulz$^{35}$,
J.~Schumacher$^{38}$,
S.J.~Sciutto$^{4}$,
A.~Segreto$^{42,44}$,
R.C.~Shellard$^{14}$,
G.~Sigl$^{39}$,
G.~Silli$^{8,36}$,
R.~\v{S}m\'\i{}da$^{36}$,
G.R.~Snow$^{89}$,
P.~Sommers$^{87}$,
S.~Sonntag$^{40}$,
J.~F.~Soriano$^{83}$,
R.~Squartini$^{9}$,
D.~Stanca$^{70}$,
S.~Stani\v{c}$^{73}$,
J.~Stasielak$^{66}$,
P.~Stassi$^{33}$,
M.~Stolpovskiy$^{33}$,
F.~Strafella$^{53,45}$,
A.~Streich$^{35}$,
F.~Suarez$^{8,11}$,
M.~Suarez Dur\'an$^{27}$,
T.~Sudholz$^{12}$,
T.~Suomij\"arvi$^{31}$,
A.D.~Supanitsky$^{5}$,
J.~\v{S}up\'\i{}k$^{30}$,
J.~Swain$^{86}$,
Z.~Szadkowski$^{68}$,
A.~Taboada$^{36}$,
O.A.~Taborda$^{1}$,
V.M.~Theodoro$^{19}$,
C.~Timmermans$^{79,77}$,
C.J.~Todero Peixoto$^{16}$,
L.~Tomankova$^{36}$,
B.~Tom\'e$^{69}$,
G.~Torralba Elipe$^{76}$,
P.~Travnicek$^{29}$,
M.~Trini$^{73}$,
R.~Ulrich$^{36}$,
M.~Unger$^{36}$,
M.~Urban$^{38}$,
J.F.~Vald\'es Galicia$^{65}$,
I.~Vali\~no$^{76}$,
L.~Valore$^{57,47}$,
G.~van Aar$^{77}$,
P.~van Bodegom$^{12}$,
A.M.~van den Berg$^{78}$,
A.~van Vliet$^{77}$,
E.~Varela$^{60}$,
B.~Vargas C\'ardenas$^{65}$,
R.A.~V\'azquez$^{76}$,
D.~Veberi\v{c}$^{36}$,
C.~Ventura$^{25}$,
I.D.~Vergara Quispe$^{4}$,
V.~Verzi$^{48}$,
J.~Vicha$^{29}$,
L.~Villase\~nor$^{64}$,
S.~Vorobiov$^{73}$,
H.~Wahlberg$^{4}$,
O.~Wainberg$^{8,11}$,
D.~Walz$^{38}$,
A.A.~Watson$^{a}$,
M.~Weber$^{37}$,
A.~Weindl$^{36}$,
M.~Wiede\'nski$^{68}$,
L.~Wiencke$^{82}$,
H.~Wilczy\'nski$^{66}$,
T.~Winchen$^{34}$, %added
M.~Wirtz$^{38}$,
D.~Wittkowski$^{34}$,
B.~Wundheiler$^{8}$,
L.~Yang$^{73}$,
A.~Yushkov$^{8}$,
E.~Zas$^{76}$,
D.~Zavrtanik$^{73,74}$,
M.~Zavrtanik$^{74,73}$,
A.~Zepeda$^{61}$,
B.~Zimmermann$^{37}$,
M.~Ziolkowski$^{40}$,
Z.~Zong$^{31}$,
F.~Zuccarello$^{55,44}$


==> icrc2017_institutions.tex <==
% created on 2017-07-06

% needs \usepackage{enumitem}
\begin{description}[labelsep=0.2em,align=right,labelwidth=0.7em,labelindent=0em,leftmargin=2em,noitemsep]
\item[$^{1}$] Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina
\item[$^{2}$] Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina
\item[$^{3}$] Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina
\item[$^{4}$] IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina
\item[$^{5}$] Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina
\item[$^{6}$] Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina
\item[$^{7}$] Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina
\item[$^{8}$] Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina
\item[$^{9}$] Observatorio Pierre Auger, Malarg\"ue, Argentina
\item[$^{10}$] Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina
\item[$^{11}$] Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina
\item[$^{12}$] University of Adelaide, Adelaide, S.A., Australia
\item[$^{13}$] Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium
\item[$^{14}$] Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil
\item[$^{15}$] Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil
\item[$^{16}$] Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil
\item[$^{17}$] Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil
\item[$^{18}$] Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil
\item[$^{19}$] Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil
\item[$^{20}$] Universidade Estadual de Feira de Santana, Feira de Santana, Brazil
\item[$^{21}$] Universidade Federal de Pelotas, Pelotas, RS, Brazil
\item[$^{22}$] Universidade Federal do ABC, Santo Andr\'e, SP, Brazil
\item[$^{23}$] Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil
\item[$^{24}$] Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil
\item[$^{25}$] Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil
\item[$^{26}$] Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil
\item[$^{27}$] Universidad Industrial de Santander, Bucaramanga, Colombia
\item[$^{28}$] Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic
\item[$^{29}$] Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic
\item[$^{30}$] Palacky University, RCPTM, Olomouc, Czech Republic
\item[$^{31}$] Institut de Physique Nucl\'eaire d'Orsay (IPNO), Universit\'e Paris-Sud, Univ.\ Paris/Saclay, CNRS-IN2P3, Orsay, France
\item[$^{32}$] Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, Paris, France
\item[$^{33}$] Laboratoire de Physique Subatomique et de Cosmologie (LPSC), Universit\'e Grenoble-Alpes, CNRS/IN2P3, Grenoble, France
\item[$^{34}$] Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany
\item[$^{35}$] Karlsruhe Institute of Technology, Institut f\"ur Experimentelle Kernphysik (IEKP), Karlsruhe, Germany
\item[$^{36}$] Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany
\item[$^{37}$] Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany
\item[$^{38}$] RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany
\item[$^{39}$] Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany
\item[$^{40}$] Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany
\item[$^{41}$] Gran Sasso Science Institute (INFN), L'Aquila, Italy
\item[$^{42}$] INAF -- Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Palermo, Italy
\item[$^{43}$] INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy
\item[$^{44}$] INFN, Sezione di Catania, Catania, Italy
\item[$^{45}$] INFN, Sezione di Lecce, Lecce, Italy
\item[$^{46}$] INFN, Sezione di Milano, Milano, Italy
\item[$^{47}$] INFN, Sezione di Napoli, Napoli, Italy
\item[$^{48}$] INFN, Sezione di Roma "Tor Vergata", Roma, Italy
\item[$^{49}$] INFN, Sezione di Torino, Torino, Italy
\item[$^{50}$] Osservatorio Astrofisico di Torino (INAF), Torino, Italy
\item[$^{51}$] Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy
\item[$^{52}$] Universit\`a del Salento, Dipartimento di Ingegneria, Lecce, Italy
\item[$^{53}$] Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy
\item[$^{54}$] Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy
\item[$^{55}$] Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy
\item[$^{56}$] Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy
\item[$^{57}$] Universit\`a di Napoli "Federico II", Dipartimento di Fisica ``Ettore Pancini``, Napoli, Italy
\item[$^{58}$] Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy
\item[$^{59}$] Universit\`a Torino, Dipartimento di Fisica, Torino, Italy
\item[$^{60}$] Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico
\item[$^{61}$] Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico
\item[$^{62}$] Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico
\item[$^{63}$] Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico
\item[$^{64}$] Universidad Michoacana de San Nicol\'as de Hidalgo, Morelia, Michoac\'an, M\'exico
\item[$^{65}$] Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico
\item[$^{66}$] Institute of Nuclear Physics PAN, Krakow, Poland
\item[$^{67}$] University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland
\item[$^{68}$] University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland
\item[$^{69}$] Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal
\item[$^{70}$] ``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania
\item[$^{71}$] Institute of Space Science, Bucharest-Magurele, Romania
\item[$^{72}$] University Politehnica of Bucharest, Bucharest, Romania
\item[$^{73}$] Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia
\item[$^{74}$] Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia
\item[$^{75}$] Universidad de Granada and C.A.F.P.E., Granada, Spain
\item[$^{76}$] Universidad de Santiago de Compostela, Santiago de Compostela, Spain
\item[$^{77}$] IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands
\item[$^{78}$] KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands
\item[$^{79}$] Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands
\item[$^{80}$] Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands
\item[$^{81}$] Case Western Reserve University, Cleveland, OH, USA
\item[$^{82}$] Colorado School of Mines, Golden, CO, USA
\item[$^{83}$] Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA
\item[$^{84}$] Michigan Technological University, Houghton, MI, USA
\item[$^{85}$] New York University, New York, NY, USA
\item[$^{86}$] Northeastern University, Boston, MA, USA
\item[$^{87}$] Pennsylvania State University, University Park, PA, USA
\item[$^{88}$] University of Chicago, Enrico Fermi Institute, Chicago, IL, USA
\item[$^{89}$] University of Nebraska, Lincoln, NE, USA
\item[] -----
\item[$^{a}$] School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom
\item[$^{b}$] Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany
\item[$^{c}$] also at Vrije Universiteit Brussels, Brussels, Belgium
\item[$^{d}$] SUBATECH, \'Ecole des Mines de Nantes, CNRS-IN2P3, Universit\'e de Nantes, France
\item[$^{e}$] Fermi National Accelerator Laboratory, USA
\item[$^{f}$] Colorado State University, Fort Collins, CO
\item[$^{g}$] now at Deutsches Elektronen-Synchrotron (DESY), Zeuthen, Germany
\end{description}

